On the Necessity and Sufficiency of Discrete-Time O'Shea-Zames-Falb Multipliers

This paper considers the robust stability of a discrete-time Lurye system consisting of the feedback interconnection between a linear system and a bounded and monotone nonlinearity. It has been conjectured that the existence of a suitable linear time-invariant (LTI) O'Shea-Zames-Falb multiplier is not only sufficient but also necessary. Roughly speaking, a successful proof of the conjecture would require: (a) a conic parameterization of a set of multipliers that describes exactly the set of nonlinearities, (b) a lossless S-procedure to show that the non-existence of a multiplier implies that the Lurye system is not uniformly robustly stable over the set of nonlinearities, and (c) the existence of a multiplier in the set of multipliers used in (a) implies the existence of an LTI multiplier. We investigate these three steps, showing the current bottlenecks for proving this conjecture. In addition, we provide an extension of the class of multipliers which may be used to disprove the conjecture.

==> Zames-Falb Multipliers for Discrete-time Systems/lure.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Aug 15 08:18:32 BST 2017
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-2.5" x-max="52.5" y-min="0" y-max="30" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(20,5);(20,5);(7.5,5);(7.5,5)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(7.5,5);(7.5,5);(7.5,22.5);(7.5,22.5)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(10,25);(10,25);(20,25);(20,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,25);(30,25);(42.5,25);(42.5,25)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(42.5,25);(42.5,25);(42.5,7.5);(42.5,7.5)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(40,5);(40,5);(30,5);(30,5)"
%	 />
%<ellipse angle-start= "0"
%	 angle-end= "0"
%	 p1= "(40,7.5)"
%	 p2= "(45,7.5)"
%	 p3= "(45,2.5)"
%	 fill-style= "none"
%	 closure= "open"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(52.5,5);(52.5,5);(45,5);(45,5)"
%	 />
%<text anchor-point= "(35,7.5)"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$e_2$
%</text>
%<text anchor-point= "(15,27.5)"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$e_1$
%</text>
%<parallelogram p1= "(20,30)"
%	 p2= "(30,30)"
%	 p3= "(30,20)"
%	 fill-style= "none"
%	 />
%<parallelogram p1= "(20,10)"
%	 p2= "(30,10)"
%	 p3= "(30,0)"
%	 fill-style= "none"
%	 />
%<text anchor-point= "(25,5)"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$\phi$
%</text>
%<text anchor-point= "(25,25)"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$G$
%</text>
%<ellipse angle-start= "0"
%	 angle-end= "0"
%	 p1= "(5,27.5)"
%	 p2= "(10,27.5)"
%	 p3= "(10,22.5)"
%	 fill-style= "none"
%	 closure= "open"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(-2.5,25);(-2.5,25);(5,25);(5,25)"
%	 />
%<text anchor-point= "(50,7.5)"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$u_2$
%</text>
%<text anchor-point= "(0,27.5)"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$u_1$
%</text>
%<text anchor-point= "(37.5,27.5)"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$y_1$
%</text>
%<text anchor-point= "(12.5,7.5)"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$y_2$
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(52.5,30)(0,0)
\linethickness{0.3mm}
\put(7.5,5){\line(1,0){12.5}}
\linethickness{0.3mm}
\put(7.5,5){\line(0,1){17.5}}
\put(7.5,22.5){\vector(0,1){0.12}}
\linethickness{0.3mm}
\put(10,25){\line(1,0){10}}
\put(20,25){\vector(1,0){0.12}}
\linethickness{0.3mm}
\put(30,25){\line(1,0){12.5}}
\linethickness{0.3mm}
\put(42.5,7.5){\line(0,1){17.5}}
\put(42.5,7.5){\vector(0,-1){0.12}}
\linethickness{0.3mm}
\put(30,5){\line(1,0){10}}
\put(30,5){\vector(-1,0){0.12}}
\linethickness{0.3mm}
\put(42.5,5){\circle{5}}

\linethickness{0.3mm}
\put(45,5){\line(1,0){7.5}}
\put(45,5){\vector(-1,0){0.12}}
\put(35,7.5){\makebox(0,0)[cc]{$e_2$}}

\put(15,27.5){\makebox(0,0)[cc]{$e_1$}}
\put(5,21){\makebox(0,0)[cc]{$-$}}

\linethickness{0.3mm}
\put(20,30){\line(1,0){10}}
\put(20,20){\line(0,1){10}}
\put(30,20){\line(0,1){10}}
\put(20,20){\line(1,0){10}}
\linethickness{0.3mm}
\put(20,10){\line(1,0){10}}
\put(20,0){\line(0,1){10}}
\put(30,0){\line(0,1){10}}
\put(20,0){\line(1,0){10}}
\put(25,5){\makebox(0,0)[cc]{$\phi$}}

\put(25,25){\makebox(0,0)[cc]{$G$}}

\linethickness{0.3mm}
\put(7.5,25){\circle{5}}

\linethickness{0.3mm}
\put(-2.5,25){\line(1,0){7.5}}
\put(5,25){\vector(1,0){0.12}}
\put(50,7.5){\makebox(0,0)[cc]{$u_2$}}

\put(0,27.5){\makebox(0,0)[cc]{$u_1$}}

\put(37.5,27.5){\makebox(0,0)[cc]{$y_1$}}

\put(12.5,7.5){\makebox(0,0)[cc]{$y_2$}}

\end{picture}


==> lure.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Aug 15 08:18:32 BST 2017
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-2.5" x-max="52.5" y-min="0" y-max="30" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(20,5);(20,5);(7.5,5);(7.5,5)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(7.5,5);(7.5,5);(7.5,22.5);(7.5,22.5)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(10,25);(10,25);(20,25);(20,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(30,25);(30,25);(42.5,25);(42.5,25)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(42.5,25);(42.5,25);(42.5,7.5);(42.5,7.5)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(40,5);(40,5);(30,5);(30,5)"
%	 />
%<ellipse angle-start= "0"
%	 angle-end= "0"
%	 p1= "(40,7.5)"
%	 p2= "(45,7.5)"
%	 p3= "(45,2.5)"
%	 fill-style= "none"
%	 closure= "open"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(52.5,5);(52.5,5);(45,5);(45,5)"
%	 />
%<text anchor-point= "(35,7.5)"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$e_2$
%</text>
%<text anchor-point= "(15,27.5)"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$e_1$
%</text>
%<parallelogram p1= "(20,30)"
%	 p2= "(30,30)"
%	 p3= "(30,20)"
%	 fill-style= "none"
%	 />
%<parallelogram p1= "(20,10)"
%	 p2= "(30,10)"
%	 p3= "(30,0)"
%	 fill-style= "none"
%	 />
%<text anchor-point= "(25,5)"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$\phi$
%</text>
%<text anchor-point= "(25,25)"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$G$
%</text>
%<ellipse angle-start= "0"
%	 angle-end= "0"
%	 p1= "(5,27.5)"
%	 p2= "(10,27.5)"
%	 p3= "(10,22.5)"
%	 fill-style= "none"
%	 closure= "open"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(-2.5,25);(-2.5,25);(5,25);(5,25)"
%	 />
%<text anchor-point= "(50,7.5)"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$u_2$
%</text>
%<text anchor-point= "(0,27.5)"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$u_1$
%</text>
%<text anchor-point= "(37.5,27.5)"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$y_1$
%</text>
%<text anchor-point= "(12.5,7.5)"
%	 fill-style= "none"
%	 text-vert-align= "center-v"
%	 text-hor-align= "center-h"
%	 text-frame= "noframe"
%	 >
%$y_2$
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(52.5,30)(0,0)
\linethickness{0.3mm}
\put(7.5,5){\line(1,0){12.5}}
\linethickness{0.3mm}
\put(7.5,5){\line(0,1){17.5}}
\put(7.5,22.5){\vector(0,1){0.12}}
\linethickness{0.3mm}
\put(10,25){\line(1,0){10}}
\put(20,25){\vector(1,0){0.12}}
\linethickness{0.3mm}
\put(30,25){\line(1,0){12.5}}
\linethickness{0.3mm}
\put(42.5,7.5){\line(0,1){17.5}}
\put(42.5,7.5){\vector(0,-1){0.12}}
\linethickness{0.3mm}
\put(30,5){\line(1,0){10}}
\put(30,5){\vector(-1,0){0.12}}
\linethickness{0.3mm}
\put(42.5,5){\circle{5}}

\linethickness{0.3mm}
\put(45,5){\line(1,0){7.5}}
\put(45,5){\vector(-1,0){0.12}}
\put(35,7.5){\makebox(0,0)[cc]{$e_2$}}

\put(15,27.5){\makebox(0,0)[cc]{$e_1$}}
\put(5,21){\makebox(0,0)[cc]{$-$}}

\linethickness{0.3mm}
\put(20,30){\line(1,0){10}}
\put(20,20){\line(0,1){10}}
\put(30,20){\line(0,1){10}}
\put(20,20){\line(1,0){10}}
\linethickness{0.3mm}
\put(20,10){\line(1,0){10}}
\put(20,0){\line(0,1){10}}
\put(30,0){\line(0,1){10}}
\put(20,0){\line(1,0){10}}
\put(25,5){\makebox(0,0)[cc]{$\phi$}}

\put(25,25){\makebox(0,0)[cc]{$G$}}

\linethickness{0.3mm}
\put(7.5,25){\circle{5}}

\linethickness{0.3mm}
\put(-2.5,25){\line(1,0){7.5}}
\put(5,25){\vector(1,0){0.12}}
\put(50,7.5){\makebox(0,0)[cc]{$u_2$}}

\put(0,27.5){\makebox(0,0)[cc]{$u_1$}}

\put(37.5,27.5){\makebox(0,0)[cc]{$y_1$}}

\put(12.5,7.5){\makebox(0,0)[cc]{$y_2$}}

\end{picture}

